3D Dual-Fusion: Dual-Domain Dual-Query Camera-LiDAR Fusion for 3D Object Detection

Fusing data from cameras and LiDAR sensors is an essential technique to achieve robust 3D object detection. One key challenge in camera-LiDAR fusion involves mitigating the large domain gap between the two sensors in terms of coordinates and data distribution when fusing their features. In this paper, we propose a novel camera-LiDAR fusion architecture called, 3D Dual-Fusion, which is designed to mitigate the gap between the feature representations of camera and LiDAR data. The proposed method fuses the features of the camera-view and 3D voxel-view domain and models their interactions through deformable attention. We redesign the transformer fusion encoder to aggregate the information from the two domains. Two major changes include 1) dual query-based deformable attention to fuse the dual-domain features interactively and 2) 3D local self-attention to encode the voxel-domain queries prior to dual-query decoding. The results of an experimental evaluation show that the proposed camera-LiDAR fusion architecture achieved competitive performance on the KITTI and nuScenes datasets, with state-of-the-art performances in some 3D object detection benchmarks categories.

==> table/kitti_lt.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{Performance of 3D-LSA versus $T$, $R$, and $K$ evaluated on KITTI \textit{val} split. "w/o 3D-LSA" indicates 3D Dual-Fusion without 3D-LSA}
\begin{tabular}{cccc}
\cline{1-4}
$T$/$R$/$K$  & Easy  & Mod   & Hard \\ 
\cline{1-4}
w/o 3D-LSA       & 92.26 & 85.66 & 83.21 \\
\cline{1-4}
2048/2.0/32          & 92.73 & 85.86 & 83.47 \\
1024/2.0/32          & \textbf{92.80} & \textbf{85.96}  & \textbf{83.62} \\
1024/1.0/32          & 92.44 & 85.48 & 83.07 \\
1024/2.0/16          & 92.59 & 85.63 & 83.33 \\
\cline{1-4}
\label{table:3dlsa}
\end{tabular}
\end{table}

